Time Series Clustering With Random Convolutional Kernels

Time series data, spanning applications ranging from climatology to finance to healthcare, presents significant challenges in data mining due to its size and complexity. One open issue lies in time series clustering, which is crucial for processing large volumes of unlabeled time series data and unlocking valuable insights. Traditional and modern analysis methods, however, often struggle with these complexities. To address these limitations, we introduce R-Clustering, a novel method that utilizes convolutional architectures with randomly selected parameters. Through extensive evaluations, R-Clustering demonstrates superior performance over existing methods in terms of clustering accuracy, computational efficiency and scalability. Empirical results obtained using the UCR archive demonstrate the effectiveness of our approach across diverse time series datasets. The findings highlight the significance of R-Clustering in various domains and applications, contributing to the advancement of time series data mining.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> pics/feature_extraction.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.65\linewidth]{pics/feature_extraction.pdf}
    \caption{The time series is convolved with N kernels, whose weights (see figure \ref{fig:kernel}) are randomly chosen. Afterwards, the proportion of positive values (PPV) of the transformed time series is calculated. As a result, the transformed data has N features with values ranging from 0 to 1.}
%    \Description{Graphical representation of the convolution and PPV operations}
    \label{fig:feature extraction}
\end{figure*}

==> pics/kernel.tex <==
%wikimedia
\begin{figure}[htp]
    \centering
    \includegraphics[width=0.7\linewidth]{pics/kernel.jpg}
    \caption{1D convolutional kernel with three weights or filters \cite{oyanedel}}
    %\Description{Graphical representation of a 1D convolutional kernel with three weights or filters}
    \label{fig:kernel}
\end{figure}

==> z0_body.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%    INTRODUCTION  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}
\label{sec:introduction}





%%%%%%%%%%%%%%% TIME SERIES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Time series}
Time is a natural concept that allows us to arrange events in a sorted way from the past to the future in an evenly distributed manner (such as days, seasons of the year or years). Data points are usually taken at successive equally spaced points in time. Based on this way of describing events, the concept of time series as a sequence of discrete data points evenly distributed arises naturally. From this perspective, time series can describe a wide range of natural and social phenomena that evolve in time. A few samples are climate and weather trends, seismic measures, stock prices, sales data, biomedical measurements, body movements or Internet traffic \cite{aghabozorgi2015time}. The study of time series involves identifying its statistical properties, including trends, seasonality, and autocorrelation, and using this information to build models for prediction and classification.





%A time series is a sequence of data points collected in time order, with each data point recorded at a specific time interval. It is a collection of observations recorded over a period of time, usually at regular intervals, to study trends and patterns in the underlying data. It is used in various fields including economics, finance, social sciences, and environmental science to analyze patterns, trends and make predictions. The study of time series involves identifying its statistical properties, including trends, seasonality, and autocorrelation, and using this information to build models for prediction and control.

%\begin{figure}[tp]
%  \centering
%  \includegraphics[width=0.95\linewidth]{{pics/wins_bars.png}}
%  \caption{Number of wins of R-clustering versus other reference algorithms in terms of clustering performance evaluated over 112 time series datasets from the UCR archive.}
%  \Description{Graph bar representing the number of wins for each algorithm in the benchmark and R-clustering}
  %\label{fig:wins_bars}
%\end{figure}

%% WHY IS TIME SERIES IMPORTANT?
%%-------------------------------------------------------------------------------------------------------------
According to \cite{yang200610}, who reviewed the work of the most active researchers in data mining and machine learning for their opinions, the problem of sequential and time series data is one of the ten most challenging in data mining. Its most relevant applications are prediction and classification (supervised or unsupervised). As for time series data availability, the significant advances in data storage, collection and processing produced during the last decades have made available a large amount of data which is growing exponentially. Unfortunately, most of this data remains unlabelled, making it useless for some critical applications such as supervised learning.

%% WHY IS TIME SERIES IMPORTANT?
%%-------------------------------------------------------------------------------------------------------------
%%-------------------------------------------------------------------------------------------------------------

%%%%%%%%%%%%%%% TIME SERIES CLUSTERING  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Time series clustering}

Given the growth rate of available data, we need scalable techniques to process it. Clustering is a solution for extracting useful information from data when the classes are not labelled and could allow a plentiful amount of available data to be processed. Clustering can be defined as the task of classifying a set of objects in different subsets with a certain logic defined in advance. Since it does not need human supervision or hand-labeling, it is considered an unsupervised technique and adequate to keep up the pace of available data.

Although time series are usually considered a collection of sorted data points in time, they can also be regarded as a single object \cite{kumar2006time} and, therefore, subject to clustering. When dealing with datasets including a significant amount of time series, clustering is especially helpful because it can help to discover patterns. Other real-world applications are anomaly and novelty detection in the case of rare patterns, and prediction or recommendation in the case of frequent patterns \cite{aghabozorgi2015time}. Some examples of such applications are web traffic anomalies \cite{lakhina2005mining} in the field of Informatics or gene classification \cite{mcdowell2018clustering} in Biology. Additionally, time series clustering can be also used as a pre-processing technique for other algorithms such as rule discovery, indexing or classification \cite{aghabozorgi2015time}.


%% INFO FROM CLASSICAL TIME SERIES CLUSTERING AND LIMITATIONS
%%-------------------------------------------------------------------------------------------------------------
%%-------------------------------------------------------------------------------------------------------------
Classical approaches to time series clustering employ parametric models to represent time series and use the estimated parameters as inputs for a clustering algorithm. Some of the most popular include autorregresive-moving-average (ARMA) models or the Hidden Markov Model. However, these techniques might not model high-dimensional and noisy real-world time-series \cite{langkvist2014review} accurately. As an alternative, the shape-based approach \cite{aghabozorgi2015time} considers the shapes of time series and matches them using appropriate time series distance measures. Shape-based algorithms require, therefore, the development of specific algorithms that deal with the complex nature of time series, which makes these methods slower than general algorithms. Finally, the feature-based methods try to extract relevant features from time series and later apply a conventional clustering algorithm. 

%% THE AUTOMATIC FEATURE EXTRACTION APPROACH
%%-------------------------------------------------------------------------------------------------------------
%%-------------------------------------------------------------------------------------------------------------
Modern feature extraction techniques work in an automated fashion. They rely on architectures consisting of kernels made of weights that are the parameters of the model that are typically learnt during the training process. These kernels convolve the input data to detect the relevant features. The success of this technique is at the heart of the Deep Learning revolution \cite{goodfellow2016deep}. The academic community has achieved substantial advances during the last decade applying this technique to the problems of image classification \cite{krizhevsky2012imagenet}, time series forecasting \cite{greff2016lstm} or time series classification \cite{ismail2019deep} among others. In the field of time series clustering, \cite{ma2019learning} have developed a convolutional model with deep autoencoders. Nevertheless, the downside is that these models require a large number of weights to work correctly and, consequently, more data and longer training times.

%% THE AUTOMATIC FEATURE EXTRACTION APPROACH WITH RANDOM KERNELS
%%-------------------------------------------------------------------------------------------------------------
%%-------------------------------------------------------------------------------------------------------------
Other authors \cite[p.~1821]{bengio2013representation} propose convolutional models with static parameters to extract features, which means faster algorithms and simpler architectures given that the number of parameters to learn is much lower. Classical methods with static parameters include hand-crafted techniques, but the need for human supervision makes them not practical to deal with the enormous amounts of available data. More modern methods propose using convolutional kernels with the weights or parameters chosen at random. For instance, \cite{jarrett2009best} show that convolutional architectures with random weights can extract relevant features from image data. More recently, \cite{dempster2021minirocket} have presented an algorithm for supervised classification of time series that first extracts time series features with random convolutional kernels and then applies a linear classifier, achieving state-of-the art results in an scalable way and much faster than other algorithms with similar performance.

More modern methods propose using convolutional kernels with the weights or parameters chosen at random. For instance, \cite{jarrett2009best} show that convolutional architectures with random weights can extract relevant features from image data. More recently, \cite{dempster2021minirocket} have presented an algorithm for supervised classification of time series that first extracts time series features with random convolutional kernels and then applies a linear classifier, achieving state-of-the art results in an scalable way and much faster than other algorithms with similar performance.

Compared to related fields such as image clustering or time series forecasting and classification, the area of time series clustering has evolved more slowly than it should, given its importance in handling the growing amount of unlabeled sequential data. As a matter of fact, the first time series clustering benchmark using the UCR archive, the most extensive and publicly available time-series catalogue, was published in 2020 \cite{javed2020benchmark}. The UCR archive \cite{dau2019ucr} is a vital tool for time series researchers, with over one thousand papers employing it. At the time of writing this work, it consists of 128 datasets of different types: devices, ECGs, motion tracking, sensors, simulated data and spectrographs. Given its essential applications, more research should be conducted to develop applications for time-series clustering.

In this sense, considering the noticeable amount of successful models based on automatic feature extraction on the one hand; and, on the other hand, the need for fast and scalable methods for clustering of time series, we develop an algorithm for clustering of time series based on automatic feature extraction, specifically using the technique of convolutional random kernel. The algorithm is called R-clustering (Random-clustering), and is a fast and scalable method for time series clustering. It transforms time series through random convolutional kernels in an enhanced data representation, then uses the new data representation to feed a clustering algorithm. We compare the performance of the R-Clustering with those from the mentioned benchmark and obtain the best results. We perform additional statistical analysis of the results, not only of the new algorithm but also of those evaluated in the benchmark, as per recommendations of the machine learning community. Finally, we prove the scalability of the algorithm for larger datasets.

 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%    RELATED WORK OR BACKGROUND  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Related Work}
\label{sec:relatedWork}

In this section, we will first review the most relevant methods for time series clustering. Then, we will focus on feature extraction methods applied to 2D and 1D data: we will examine general applications and differentiate between those based on learnable kernels and those found in static kernels. Finally, we will consider applying the latter to time series clustering.


\subsection{Time Series Clustering}

%%Three aproaches
%%Model-based
Different approaches to the clustering of time series, according to \cite{aghabozorgi2015time}, can be classified in three groups: model-based, shape-based and feature-based. In the model-based methods, the time series are adjusted to a parametric model; since the parameters do not have a time series structure, a universal clustering algorithm is applied. Some popular parametric models are autorregresive-moving-average (ARMA) models or the Hidden Markov Model. However, these techniques might not accurately model high-dimensional and noisy real-world time-series \cite{langkvist2014review}. Existing methods that may address the noise issue, such as wavelet analysis or filtering, often include lag in the processed data, reducing the prediction accuracy or the ability to learn significant features from the data \cite{yang200610}.

%%shape-based
In the shape-based approach, the clustering algorithm is applied directly to the time series data with no previous transformation. Contrary to the model-based approach, these methods employ a clustering method with a similarity measure appropriate for time series. For example, \cite{paparrizos2015k} introduce the k-shape algorithm with a shape-based approach. In their work, the authors suggest that feature-based strategies are not convenient because they are domain dependent and require modification of the algorithms when used on different datasets. Another shape-based method is to apply an universal clustering algorithm, commonly the k-means algorithm \cite{macqueen1967classification}, with an appropriate distance measure that takes into account the peculiarities of time series, such as dynamic time warping (DTW), introduced by \cite{berndt1994using}. Although it has been established that DTW performs better for time series clustering, the drawback is it has a time complexity of \begin{math} \mathcal{O}(n^2) \end{math}, where n is the length of time series. Compared to DTW, the Euclidean distance, which is the distance usually used in the k-means algorithm \cite{likas2003global}, has a complexity of \begin{math} \mathcal{O}(n) \end{math} \cite{jain1999data}.


%%Feature-based
Feature-based methods first extract relevant time series features and later apply a conventional clustering algorithm \cite{aghabozorgi2015time}. As we will see in the next section, feature-based algorithms have been proven quite successful for image clustering and classification. According to \cite[p.~1798]{bengio2013representation}, the performance of machine learning algorithms relies strongly on the correct choice of feature representation.




\subsection{Feature extraction}
%%%% Manual feature extraction %%%%
Prior research confirms that incorporating expert knowledge helps Machine Learning, as \cite{bengio2013representation} and \cite{sebastiani2002machine} show. The most prevalent way for years to achieve so has been to hand design feature extractors that feed a generic classifier as in \cite{lowe1999object}. However, developing tools by hand that capture the relevant information for each task is time-consuming and requires expert human supervision, which is only sometimes available. Additionally, the exponential growth of the available data demands scalable feature extraction techniques.

%%%% Automatic feature extraction %%%%
In some domains, such as the 2D shape of pixels in images or time series having a 1D structure, it is possible to learn better features using only a basic understanding of the input as an alternative to incorporating expert knowledge. In images and time series data, patterns are likely to reproduce at different positions, and neighbours are likely to have strong dependencies. The existence of such local correlations is the basis for applying a local feature extractor all over the input and transforming it into a feature map of a similar structure. A convolution operation usually performs this task with a convolutional kernel \cite[p.~1820]{bengio2013representation}. In the figure \ref{fig:kernel} a kernel consisting of three weights (or filters) convolves one-dimensional input data.% En series temporales, evidentemente hay efectos periódicos no locales.




%wikimedia
\begin{figure}[htp]
    \centering
    \includegraphics[width=0.8\linewidth]{pics/kernel.png}
    \caption{1D convolutional kernel with three weights or filters \cite{oyanedel}}
    %\Description{Graphical representation of a 1D convolutional kernel with three weights or filters}
    \label{fig:kernel}
\end{figure}

%%%%%%%%%%%%%%% LEARNABLE FEATURE EXTRACTION  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%% ¿¿o simplemente learnable kernels??  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Feature extraction with learnable kernels}

In most convolution algorithms, kernel weights are typically learnt during the training process \cite{bengio2013representation}. Over the last few years, the academic community has extensively explored the applications of such convolutional models for image classification and segmentation. See \cite{ciresan2011flexible}, \cite{pereira2016brain}, \cite{krizhevsky2012imagenet}. %In these works, neural networks with convolutional layers transforms the image data arriving at a final representation with a small number of variable. The last step of the architecture is a linear classification algorithm over these variables.


%% LEARNABLE FEATURE EXTRACTION FOR IMAGE CLUSTERING
%%-------------------------------------------------------------------------------------------------------------
Some authors have applied convolutional architectures to the problem of image clustering \cite{caron2018deep},  \cite{xie2016unsupervised}. Both models presented in these papers consist of a network that transforms the input data into an enhanced feature representation, after which a clustering algorithm is applied. In both cases, a learning process jointly optimizes the network weights and the clustering parameters. The first model predicts the label of the inputs based on the clustering prediction and then backpropagates the prediction error to adjust the network parameters. The second model incorporates an autoencoder with a bottleneck in the middle and a learning algorithm with two steps. First, the network parameters are optimized using the reconstruction loss. Afterwards, the decoder part of the architecture is discarded, and the output features at the bottleneck make up the new data representation which is the input for a clustering algorithm.


%% LEARNABLE FEATURE EXTRACTION FOR TIME SERIES CLASSIFICATION
%%-------------------------------------------------------------------------------------------------------------
Other authors have developed models based on convolutions with learnable weights to process time series data, such as convolutional autoencoders or convolution Restricted Boltzmann Machines \cite{langkvist2014review}. More recently, \cite{ismail2019deep} used convolutional neural networks for time series classification achieving state-of-the-art results. 




%% LEARNABLE FEATURE EXTRACTION FOR TIME SERIES CLUSTERING
%%-------------------------------------------------------------------------------------------------------------
\cite{ma2019learning} have recently presented a clustering algorithm for time series that combines previous image clustering techniques. On the one hand, the model gets a reconstruction loss from an autoencoder. On the other hand, it predicts the labels according to a clustering layer from which a prediction loss is obtained. The model combines both losses to optimize the parameters of the network jointly with the clustering parameters.

%%%% Problems %%%%
These works show that the convolution operation with learnable kernels is a compelling image and time series processing technique. As a drawback, the families of models using convolution with learnable weights require architectures with several layers and a significant number of parameters to work optimally \cite{bengio2013representation}, \cite{goodfellow2016deep}. Since the parameters need to be optimized during the learning process, the more parameters the architecture has, the longer the training process and the more data are required.

%% FEATURE EXTRACTION WITH LEARNABLE KERNELS
%%-------------------------------------------------------------------------------------------------------------
%%-------------------------------------------------------------------------------------------------------------
\subsubsection{Feature extraction with random kernels}

From a different perspective, some authors \cite[p.~1821]{bengio2013representation} propose convolutional models with static parameters to extract features, which means faster algorithms and simpler architectures since the training process that optimizes the parameters is no longer necessary. The question is whether these models achieve enhanced feature representations. \cite{lowe1999object} proposes an algorithm for image feature extraction where static filters are built by hand to attain specific invariances in the transformed data. Although the model achieves remarkable results, the impossibility of automating this process makes it unfeasible to process the amount of available data. Other authors propose using static parameters whose values are chosen at random: \cite{huang2014insight}, \cite{jarrett2009best} show that convolutional architectures with random weights can extract relevant features from data in the context of image recognition. \cite{saxe2011random} prove that choosing the right network design is, in some cases, more relevant in terms of algorithm accuracy than choosing between random or learnable weights. They also conclude that convolutional architectures with random kernels are frequency selective, justifying the use of such structures for time series analysis.

%%%% Random filters for feature extraction of time series (pipeline) %%%%

%%%%%%%%%%%%%%%%%%%% PIPELINE - TODO %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
More recently, \cite{dempster2021minirocket} have presented Minirocket, a model with such an architecture for supervised classification of time series. The model transforms the input data with convolutional random kernels; then, the transformed data are used to train a linear classifier (ridge regression classifier or logistic regression for larger datasets). The study evidences that using such kind of random kernels rather than learnable kernels can be a great advantage. The computational needs are fewer, and algorithms are much faster while obtaining similar or even better performance. Figure \ref{fig:feature extraction} shows a schema of feature extraction of a time series with random kernels based on the work by \cite{dempster2021minirocket}. Minirocket achieves state-of-the-art results in a more scalable way than other algorithms for the problem of supervised classification of time series, showing that random kernels is an effective and efficient technique for time series processing.

%It seems natural to expect that transformation of a time series with random kernels, due to the random nature of its weights, produces uncorrelated data and removes temporal regularities. We have performed some experiments with the original code of the Minirocket algorithm to test that hypothesis, but after examining the original transformation using the publicily available code of the algorithm, we have found periodic signals in the ouput, contrary to our expectations. See figure XXX.

%Despite this issue, 

%%Existing methods for time series classification typically focus on a single repre- sentation such as shape, frequency, or variance. Convolutional kernels constitute a single mechanism which can capture many of the features which have each previ- ously required their own specialized techniques, and have been shown to be effec- tive in convolutional neural networks for time series classification such as ResNet (Wang et al. 2017; Ismail Fawaz et al. 2019a), and InceptionTime. (ROCKET) %

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.65\linewidth]{pics/feature_extraction_vertical_vf.png}
    \caption{The time series is convolved with N kernels, whose filters (see figure \ref{fig:kernel}) are randomly chosen. Afterwards, the proportion of positive values (PPV) of the transformed time series is calculated. As a result, the transformed data has N features with values ranging from 0 to 1.}
%    \Description{Graphical representation of the convolution and PPV operations}
    \label{fig:feature extraction}
\end{figure*}


%Paparrizos Several methods have been proposed to cluster time se- ries. All approaches generally modify existing algorithms, either by replacing the default distance measures with a version that is more suitable for comparing time series (raw- based methods), or by transforming the sequences into “flat” data so that they can be directly used in classic algorithms (feature- and model-based methods) [83]. Raw-based ap- proaches can easily leverage the vast literature on distance measures (see Section 2.3), which has shown that invari- ances offered by certain measures, such as DTW, are gen- eral and, hence, suitable for almost every domain [19]. In contrast, feature- and model-based approaches are usually domain-dependent and applications on different domains re- quire that we modify the features or models. Because of these drawbacks of feature- and model-based methods, in this paper we follow a raw-based approach.

 

% THERE IS A GAP: RANDOM FEATURE EXTRACTION FOR TIME SERIES CLUSTERING (feature bases method using random kernels!! 


%%Salvador: Euclidean distance is an efficient distance measurement that can be used. The Euclidian distance between two time series is simply the sum of the squared distances from each nth point in one time series to the nth point in the other. The main disadvantage of using Euclidean distance for time series data is that its results are very unintuitive. If two time series are identical, but one is shifted slightly along the time axis, then Euclidean distance may consider them to be very different from each other. Dynamic time warping (DTW) was introduced [11] to overcome this limitation and give intuitive distance measurements between time series by ignoring both global and local shifts in the time dimension.



%dtw better than euclidean: http://alumni.cs.ucr.edu/~ratana/KAIS04.pdf

Motivated by the success of random kernels applied to the problem of feature extraction of time series and image data, we propose a simple and fast architecture for time series clustering using random kernels. To our knowledge, convolutional architectures with random weights for time-series clustering have never been tested before. With such an architecture, it is not necessary to reconstruct the input with a decoder to get a reconstruction loss, or to build a classifier and obtain a classification loss to adjust the parameters, as in the works about time-series clustering mentioned before. The new method applies the convolution operation with random filters over the time series input data, obtaining an enhanced feature representation. The transformed data feed a K-means clustering algorithm. We have conducted several experiments to test the effectiveness and scalability of the algorithm, improving current state-of-the-art results. 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%    METHODS  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Methodology}
\label{sec:methods}

This section explains the proposed clustering algorithm and the evaluation methods, including a statistical analysis.

%%Clustering Algorithm
\subsection{Clustering algorithm}

We present a new algorithm for time series clustering, called R-clustering which is composed of two data processing elements connected in series. The first element is a feature extractor made up of convolutional random kernels, which transforms the input time series in an enhanced data representation. The second processing element is a K-means algorithm \cite{macqueen1967classification} with Euclidean distance that provides the clustering capabilities.


%The first phase of the method consists of extracting features from time series data input using convolutional random kernels and then applying the PPV operation. The feature extracted is based on the one used in \cite{dempster2021minirocket} with improvements.The second phase of the algorithm consists of a classic clustering algorithm whose input is the transformed data.

%As explained in last section, the time series is convolved with kernels whose filters are sampled at random. Afterwards, the proportion of positive values (PPV) of the transformed time series is calculated. As a result, if the number of kernels is N, the transformed data has N features with values ranging from 0 to 1. Due to the randomness introduced in the weights, it seems likely that the output of this data transformation, i.e., the N features, do not inherit temporal correlations from the input time series. However, we have analyzed the output for several time series from the UCR dataset and found temporal correlations in all of them, as we will see in the results section.

%After examining the original transformation, we have found some regularities in its design that could be the cause of the temporal correlations. We have modified the original transformation introducing random permutations to the output data to remove the regularities. We will refer to this transformation as the modified transformation. After this change, the output data does not present time series characteristics anymore and can be considered raw data, following the terminology of \citet{aghabozorgi2015time}. Due to this change in the nature of the data, a universal clustering algorithm becomes more convenient than a time-series-specific one.

%%first phase
\subsubsection{First phase of the algorithm: feature extraction}
\label{subsec:feature_extraction}
For this first stage of the algorithm, we start with the configuration of the feature extractor present in Minirocket \cite[p.~251]{dempster2021minirocket}. We use 9,996 kernels of length 9, whose weights values are randomly chosen from -1 or 2. To select the bias values, fist each kernel is convolved with a time series selected at random from the dataset. Then, the algorithm draws the bias values from the quantiles of the result. The number of dilations are a fixed function of the input length and padding is fixed. After the convolution of the input series with these kernels, the proportion of positive values (PPV) of the resulting series is calculated. Therefore, under this configuration, the transformed data consists of 9,996 features with values between 0 and 1. %AQUÍ 29-1

Despite the good results shown by Minirocket, a thorough examination of the output of the feature extractor stage reveals there are artificial autocorrelations, not from the time series data,  produced by the implementation of the algorithm. This behaviour could affect the performance of the clustering stage of R-clustering, or of a future algorithm using this feature extractor, because it would likely detect these unnatural patterns. Also, these patterns could mask legit features of time series, obtaining misleading results. We have identified that the quantiles mentioned above from which the algorithm draws the bias values, are sorted from high to low values, producing artificial patterns in the output. Consequently, we have modified the feature extractor by introducing random permutations in the quantiles. By implementing this change, we have managed to remove artificial autocorrelations. (see \ref{subsec:RK-transformation} for a detailed description of the output of the feature extractor after and before the modifications)

\begin{figure*}[h]
    \centering
    \includegraphics[width=0.85\linewidth]{pics/RKC-schema_V2.png}
    \caption{Schema of the R-clustering algorithm with its stages: 1) 9,996 random kernel convolve the same input time series. The PPV operation is applied to the result of the convolution, obtaining 9,996 features ranging from 0 to 1. 2) The 9,996 features make up a new time series that represents a data point. 3) The data points from all the transformed time series of a dataset are clustered with the K-means algorithm with Euclidean distance.}
%    \Description{Figure represents the stages of the R-clustering algorithm }
    \label{fig:rkc-schema}
\end{figure*}

%%second phase TODO
\subsubsection{Second phase of the algorithm: K-means with Euclidean distance}
%As proven, the transformed data can be considered as raw-data in a relevant proportion; therefore, it makes more sense to use a universal clustering algorithm rather than one specific for time series such as DTW or one based in shaped based distance.
For the second stage of R-clustering, we use a universal clustering algorithm: the K-means algorithm \cite{macqueen1967classification} with Euclidean distance, a combination that the scientific community has already tested in the context of clustering problems: \cite{jain1999data}, \cite{likas2003global}. K-means partitions data into a number K (set in advance) of clusters by iteratively assigning each data point to the \emph{nearest} mean center (centroid) of a cluster. After each new assignment, the centroids are recalculated. When the training process finishes, the resulting centroids can be used to classify new observations. Note that a distance must be defined to evaluate the \emph{nearest} centroid in each step of the algorithm. As mentioned before, using the Euclidean distance will result in a more efficient algorithm since it has a time complexity of \begin{math} \mathcal{O}(n) \end{math}. In contrast, if we used DTW as a distance for K-means, the time complexity would be of \begin{math} \mathcal{O}(n^2) \end{math}. See figure \ref{fig:rkc-schema} for a schema of the R-clustering algorithm with all its phases.

%minirocket abstract: by transforming input time series using random convolutional kernels, and using the transformed features to train a linear classifier.



%% IDEA: BUSCAR EL ARTÍCULO QUE DICE QUE ED VS DTW NO ES TAN DIFERENTE Y USAR ED POR SIMPLICIDAD. DTW INTRATABLE %%

%% TODO: CHECK THAT THE TRANSFORMED DATA IS RAW DATA, IE, IT IS NOT CORRELATED (SAMPLES ARE IID??)
%%-------------------------------------------------------------------------------------------------------------
%langkvist tiene una buena introducción sobre las características de las series temporales. Quizás uno de los libros que tengo en icloud?

%Papparizos 2.2 talks about time-series invariances. We could maybe compare them to kernel processed data to check whether they can still be considered time series. 2.3 speaks about time series distance measures that should account for time series invariances. If we eliminate invariances, we no longer need complicated measures that account for them.

%Idea: permutamos los datos (las coordenadas) de la serie temporal y de los transformados y comprobamos si los resultados son los mismos. (Hacemos una permutación de las coordenadas, por igual en todas las series. En la definición del ECUMV en estadística)

%Sencillo: Ljung Box Test para ver si hay autocorrelaciones.


%% TODO: EXPLAIN FURTHER OUR ALGORITHM
%%-------------------------------------------------------------------------------------------------------------
%%It uses the most famous and extensive time-series dataset, the publicly available UCR \cite{dau2019ucr} time series archive.



\subsection{Evaluation method}
To the authors' knowledge, the only benchmark for time series clustering using the widely used UCR dataset is the one presented by \cite{javed2020benchmark}. This benchmark compares eight popular clustering methods that cover three categories of clustering algorithms (partitional, density-based, and hierarchical) and three distance measures (Euclidean, Dynamic time warping, and shape-based). We assess the performance of R-clustering on the same 112 datasets from the UCR archive as the benchmark (16 out of 128 datasets are not used, 11 of them because they have varying lengths, and 5 because they have only one class). To guarantee a fair comparison of results, we evaluate the performance of our algorithm following the same procedures described in the benchmark. Because the UCR archive is labelled, the number of clusters of each dataset is known in advance. Therefore, this number is used as an input for the clustering algorithms in the benchmark as in our work. Different methods exist to estimate the number of clusters, such as the elbow method \cite{thorndike1953belongs}. However, evaluating these methods is not a part of the benchmark or this paper.

Several metrics help to evaluate a clustering process, such as Rand Index (RI) \cite{rand1971objective}, Adjusted Mutual Information \cite{vinh2009information} or Adjusted Rand Index (ARI) \cite{hubert1985comparing}.  ARI is a similarity measure used to compare two clustering results of a given set of objects that considers the chance assignment of clusters. It is based on the Rand Index but is adjusted for randomness. As the benchmark we are following illustrates, ARI is independent of the number of clusters, in contrast to non-adjusted measures such as RI, that show dependence on the number of clusters. \cite{steinley2004properties} also supports choosing the ARI metric to evaluate clustering performance above other metrics. Based on these reasons and for comparability with the benchmark, we use the Adjusted Rand Index (ARI) to evaluate R-clustering.

To compare the performance of the algorithms, we use the same methods as in the benchmark study: we calculate the number of datasets for which an algorithm obtains the highest ARI (number of wins), the mean ARI score and the mean rank among all the algorithms of the benchmark across the same 112 datasets. Under all comparison methods, the R-clustering improves the results of the rest of the algorithms.  

%we report the number of datasets (called ‘‘winning count’’) for which an algorithm or a distance measure achieved the highest ARI, 

%%%%%%%%%%%%%%%%  Statistical Analysis %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Statistical analysis} / WE DELETE THIS SUBSECTION HEADER-
Another relevant question, not present in the benchmark study, is whether there are statistical significant differences between algorithms in their performance. The problem of comparing multiple algorithms over multiple datasets in the context of machine learning has been treated by several authors \cite{demvsar2006statistical}, \cite{garcia2008extension}, \cite{benavoli2016should}. Following their recommendations, we first compare the ranks of the algorithms as suggested by \cite{demvsar2006statistical} and use the Friedman test to decide whether there are significant differences among them. If the test rejects the null hypothesis (i.e., "there are no differences"), we try to establish which algorithms are responsible for these differences. As \cite{garcia2008extension} indicates, after the Friedman test rejects the null hypothesis, we should proceed with another test to find out which algorithms produce the differences through pairwise comparisons. Following the recommendations of the authors of the UCR Dataset,  \cite{dau2019ucr}, we will use the Wilcoxon sign-test for the pairwise comparisons between the R-clustering algorithm and the rest. As detailed in Section \ref{sec:results}, we first compare the R-clustering algorithm with the rest of the algorithms included in the benchmark and determine which ones present significant differences. In addition, \cite{garcia2008extension} recommends performing all pairwise comparisons in experimental works, not only with the new methods, but also between existing ones. Consequently, we repeat the pairwise comparisons for each of the algorithms in the benchmark. The results will complement the conclusions of the benchmark with more robust statistical analysis.




\subsection{Implementation and reproducibility}
We use Python 3.6 software package on Windows OS with 16GB RAM, Intel(R) Core(TM) i7-2600 CPU 3.40GHz processor for their implementation. Besides standard Python libraries, we use the library sktime \cite{loning2019sktime} for evaluating the computation time of the Agglomerative algorithm, the code available in  \cite{paparrizos2015k} for evaluating the computation time of the K-shape algorithm, scikit-learn \cite{scikit-learn} for executing the K-means stage of R-clustering and for evaluating the adjusted rand index and the functions provided in \cite{ismail2019deep} for calculating the statistical results. The code will be made publicly available, and we use a public dataset to ensure the full reproducibility of the experiment

%The code will be made publicly available  \footnote{the code will be available after the review, or before upon request}, and we use a public dataset to ensure the full reproducibility of the experiments.  


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  RESULTS  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Results}
\label{sec:results}
In this section, we first present the analysis of the output after the feature extractor stage mentioned in \ref{subsec:feature_extraction}. Then, we offer the results of the R-clustering algorithm on 112 datasets of the UCR archive and compare them to the results of the algorithms evaluated on the reference benchmark. Finally, we describe the conclusions of a complete statistical analysis of the R-clustering and the rest of the algorithms.

\subsection{Configuration of the feature extractor}
\label{subsec:extractor-configuration}
 
\subsection{Output of the feature extractor}
\label{subsec:RK-transformation}

Figure \ref{fig:fungi-sample} shows a sample time series from the UCR archive, and figure \ref{fig:transformed_fungi} (left) shows the transformation of this time series with the original feature extractor, where the existence of autocorrelations is evident. However, we analyze the autocorrelation properties with a Ljung-Box test, whose null hypothesis is that no autocorrelations exist at a given lag. As expected after observing figure \ref{fig:transformed_fungi} (left), the test has rejected the null hypothesis for every lag at a confidence level of 95\%, so we assume that autocorrelations exist. To test whether these periodic properties originate in the time series data, we introduce noisy data in the feature extractor and repeat the Ljung-Box test. We obtain autocorrelations again at every lag. Therefore, we conclude that the original feature extractor raises artificial autocorrelations, not from the input time series. After modifying the implementation (see details in the codeas explained in \ref{subsec:feature_extraction}, we introduce the same noisy data and repeat the Ljung-Box test. This time, the test does not reject the null hypothesis at any lag, so it is not unsafe to assume that no autocorrelations exist and that the feature extractor works as expected, that is, producing noisy data from noisy data. For a sample transformation of a time series with the new feature extractor see Figure \ref{fig:transformed_fungi} (right) 


\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{pics/fungi_sample.png}
%    \Description{Sample time-series from Fungi dataset included in the UCR archive }
    \caption{Sample time-series from Fungi dataset included in the UCR archive. The dataset contains high-resolution melt curves of the rDNA internal transcribed spacer (ITS) region of 51 strains of fungal species. The figure shows the negative first derivative (-dF/dt) of the normalized melt curve of the ITS region of one of such species}
    \label{fig:fungi-sample}
\end{figure}
\begin{figure*}[t]
  \begin{subfigure}[b]{0.47\linewidth}
    \includegraphics[width=\textwidth]{pics/transformed_fungi_original.png}
    %\caption{transformed time series with the original Minirocket algorithm}
    \label{fig:transformed_fungi_original}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.47\linewidth}
    \includegraphics[width=\textwidth]{pics/transformed_fungi_modified.png}
    %\caption{Sample time-series from Fungi dataset included in the UCR archive}
    \label{fig:transformed_fungi_modified}
  \end{subfigure}
%  \Description{Transformed time series from Fungi dataset  with the original feature extractor from Minirocket algorithm and the modified feature extractor. Y axis shows the calculated PPV after the convolution}
  \caption{Transformed sample time-series from Fungi dataset (figure \ref{fig:fungi-sample}) with the original feature extractor from Minirocket algorithm (left) and the modified feature extractor (right)}
  \label{fig:transformed_fungi}
\end{figure*}


\subsection{Dataset-level assessment}
We evaluate R-clustering on the same 112 datasets from the UCR archive chosen in \cite{javed2020benchmark}. As explained, R-clustering uses the K-means algorithm with Euclidean distance, which is an optimization np-hard problem \cite{aloise2009np}. Since finding a global optimum is complex, the algorithm is often run several times with different random centroids initialization to improve the performance. Finally, the best score (best local optimum) of all runs is chosen. This study uses the same procedure as the benchmark: the results are scores over ten runs. The K-means algorithm needs the number of clusters in advance to run. Different methods exist to estimate it, such as the elbow method \cite{thorndike1953belongs}, but evaluating these methods is not a part of the benchmark. Since we are using a labelled dataset in this experiment, the R-clustering algorithm receives the target number of clusters as input. 


%% JAVED: Known number of clusters. The clustering methods used in this work require that the number of clusters, k, be provided as input. The value of k is known from the class labels annotated in the datasets. There are several techniques for estimating k (e.g., Bezdek & Pal, 1998; Bholowalia & Kumar, 2014; Patil & Baidari, 2019; Subbalakshmi et al., 2015), but evaluating those techniques is not part of this benchmark.
%%

%% TODO: EXPLAIN THAT IN REAL APPLICATIONS WE DON'T HAVE THE CLUSTERS
%%--

%%%%%%%%%%%%%%%%  R-clustering Algorithm Results %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Results of the R-clustering algorithm}
We compare the performance of R-clustering to the other algorithms of the benchmarks over the 112 datasets under several perspectives using the ARI metric. We count the number of wins considering that ties do not sum and calculate the mean score and rank. R-clustering obtains the highest number of wins (39) followed by k-shape (21) (see table \ref{winning_counts}), the best mean rank (3.67) followed by k-means-DTW (4.53) (see table \ref{mean_rank}), and the best mean ARI score (0.277) followed by Agglomerative (0.259) (see figure \ref{fig:aris})



%Valores R-clustering_API_PERM   
\begin{table}[t]
\centering
\caption{number of wins for each algorithm over 112 datasets in terms of best ARI}
\begin{tabular}{lr}
\toprule
algorithm &   Winning count \\
\midrule
R-clustering                         & 39 \\
K-shape                     & 21 \\
Density Peaks (DTW)         & 13 \\
K-means (DTW)               & 11 \\
Agglomerative (Euclidean)   & 10 \\
C-means (Euclidean)         &  5 \\
Density Peaks (Euclidean)   & 4 \\
K-means (Euclidean)         & 3 \\
K-medoids (Euclidean)       & 1 \\
\bottomrule
\end{tabular}
\label{winning_counts}
\end{table}


\begin{table}[h]
\centering
\caption{mean rank for R-clustering and the rest of the algorithms considered in the benchmark}
\begin{tabular}{lr}
\toprule
Algorithm &   Mean rank \\
\midrule
R-clustering                       &  3.67 \\
K-means (DTW)             &  4.53 \\
K-means (Euclidean)       &  4.54 \\
K-shape                   &  4.54 \\
Agglomerative (Euclidean) &  4.57 \\
C-means (Euclidean)       &  5.32 \\
K-medoids (Euclidean)     &  5.51 \\
Density Peaks (Euclidean) &  6.12 \\
Density Peaks (DTW)       &  6.17 \\
\bottomrule
\end{tabular}
\label{mean_rank}
\end{table}


\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\linewidth]{pics/aris.png}
    \caption{Average ARI for each algorithm over 112 datasets}
%    \Description{bar graph showing the results of the algorithms of the benchmark evaluated over 112 datasets}
    \label{fig:aris}
\end{figure}






%We analyzed CID and Euclidean distance results using the Wilcoxon signed-ranks test. This is the statistical test recommended by Demšar (2006) to compare two algo- rithm over multiple data sets. The test indicates that the null-hypothesis, i.e. both distances have the same performance, should be rejected with 95 % confidence level. Therefore, CID outperforms Euclidean distance with statistical significance. (https://www.researchgate.net/profile/Vinicius-Alves-De-Souza/publication/254861501_CID_An_efficient_complexity-invariant_distance_for_time_series/links/0deec51fe65bc20dfa000000/CID-An-efficient-complexity-invariant-distance-for-time-series.pdf)

In addition, we perform a statistical comparison of R-clustering with the rest of the algorithms following the recommendations of \cite{dau2019ucr} and \cite{demvsar2006statistical}, that suggest to compare the rank of the classifiers on each dataset. First, we perform the Friedman test \cite{friedman1937use} with a 95\% confidence level, that rejects the null hypothesis of no difference among all the algorithms. As per \cite{benavoli2016should} recommendations, since the test rejects the null hypothesis, we need to find out which are the significant differences among the algorithms. To achieve this, we perform a pairwise comparison of R-clustering versus the rest of the classifiers using the Wilcoxon signed-rank test with a 95\% confidence level, including the Holm correction, which adjusts family-wise error. We can summarize the statistical rank analysis of as follows. R-clustering is the best-performing algorithm, with an average rank of 3.67. The pairwise comparisons manifest that R-clustering presents significant differences, in terms of mean rank, with all algorithms except with K-shape, and Agglomerative. 







%https://tex.stackexchange.com/questions/163061/help-with-a-booktabs-table
%https://lazyscientist.wordpress.com/2021/07/23/make-better-tables-in-latex-using-booktabs/
%https://nhigham.com/2019/11/19/better-latex-tables-with-booktabs/
%R-clustering stands for random kernel clustering






\begin{figure*}[t]
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pics/length_ducks_geese.png}
    %\caption{transformed time series with the original Minirocket algorithm}
    \label{fig:scalability_l}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.49\textwidth}
    \includegraphics[width=\textwidth]{pics/size_insect_sound.png}
    %\caption{Sample time-series from Fungi dataset included in the UCR archive}
    \label{fig:scalability_s}
  \end{subfigure}
  \caption{Scalability of R-clustering and the rest of the 3 best performing algorithms with respect to the number of time series in the dataset (left) and the length of the time series of the dataset (right)}
%  \Description{line graph representing the compute time of the 3 best performing algorithm for a variable size.}
  \label{fig:scalability}
\end{figure*}

\subsection{Compute Time and Scalability}
% ROCKET: The total compute time (training and test) for Rocket on all 85 ‘bake off’ datasets is 1 hour 50 minutes, compared to more than 6 days for InceptionTime (trained and tested using GPUs), Other recent methods that do not deal with feature extraction and need to use complicated methods for clustering techniques, while feature extraction allow to use classical and more tested clustering methods. Is shape-based algorithm scalable?


% KSHAPE: 4 horas 43 Mins
% Agglomerative: 8 Mins, 15 secs.
% R-clustering: 43 minutos

In this subsection, we compare the compute time and scalability of the R-clustering algorithm to the algorithms with which it does not present significant differences in terms of mean rank: K-shape and Agglomerative. The total compute time for R-clustering on all 112 datasets is 43 minutes, for K-shape is 4 hours 32 minutes, and for the Agglomerative algorithm is 8 minutes. However, it is important to note that time complexity of Agglomerative is \begin{math} \mathcal{O}(n^2) \end{math}  \cite{de2004open} and requires \begin{math} \mathcal{O}(n^2) \end{math} memory \cite{murtagh1984complexities} so it may cause computation problems for larger datasets and may not scale properly, as the following experiment will show.

For the scalability study, we use two recent datasets not used in the benchmark: DucksAndGeese and InsectSound. DucksAndGeese has a size of 100 time series, 5 classes and is the longest dataset in the archive with a length of 236,784 points. InsectSound has a size of 50,000 time series, each of which has a length of 600 points and 5 classes. The results are represented in figure \ref{fig:scalability}, that shows the scalability of R-clustering in terms of time series length and time series size. R-clustering scales linearly with respect to both: the length of the time series of the dataset (length of the dataset) and the number of time series in the dataset (size of the dataset). For a moderate size of the dataset, Agglomerative is the fastest algorithm even for long time series. However, when the size of the dataset grows, R-clustering becomes the fastest algorithm of the three.





\begin{table*}[t]
\centering
%Begin latex from Pandas

\begin{tabular}{lllc}
\toprule
              Algorithm 1 &               Algorithm 2 &      p value &  Significant difference \\
\midrule
Density Peaks (Euclidean) &                       R-clustering & 2.939982e-08 &                    True \\
      K-means (Euclidean) &     K-medoids (Euclidean) & 7.516924e-08 &                    True \\
      Density Peaks (DTW) &                       R-clustering & 3.651556e-07 &                    True \\
Agglomerative (Euclidean) &     K-medoids (Euclidean) & 1.183446e-06 &                    True \\
    K-medoids (Euclidean) &                       R-clustering & 6.988398e-06 &                    True \\
      Density Peaks (DTW) &             K-means (DTW) & 9.209253e-06 &                    True \\
Agglomerative (Euclidean) &       Density Peaks (DTW) & 1.863177e-05 &                    True \\
Density Peaks (Euclidean) &       K-means (Euclidean) & 4.440957e-05 &                    True \\
      Density Peaks (DTW) &       K-means (Euclidean) & 7.363479e-05 &                    True \\
      C-means (Euclidean) &                       R-clustering & 9.099955e-05 &                    True \\
Agglomerative (Euclidean) & Density Peaks (Euclidean) & 1.541735e-04 &                    True \\
      K-means (Euclidean) &                       R-clustering & 1.910857e-04 &                    True \\
Density Peaks (Euclidean) &             K-means (DTW) & 2.032777e-04 &                    True \\
      Density Peaks (DTW) &     K-medoids (Euclidean) & 5.362103e-04 &                    True \\
Agglomerative (Euclidean) &       K-means (Euclidean) & 6.785202e-04 &                    True \\
            K-means (DTW) &     K-medoids (Euclidean) & 6.857564e-04 &                    True \\
            K-means (DTW) &                       R-clustering & 1.207988e-03 &                    True \\
Agglomerative (Euclidean) &       C-means (Euclidean) & 1.264458e-03 &                    True \\
Density Peaks (Euclidean) &                   K-shape & 1.682662e-03 &                    True \\
      C-means (Euclidean) &       K-means (Euclidean) & 2.149903e-03 &                    True \\
      C-means (Euclidean) &             K-means (DTW) & 2.312641e-03 &                    True \\
                  K-shape &                       R-clustering & 4.440235e-03 &                   False \\
      Density Peaks (DTW) &                   K-shape & 4.906171e-03 &                   False \\
Agglomerative (Euclidean) &                       R-clustering & 1.117005e-02 &                   False \\
Density Peaks (Euclidean) &     K-medoids (Euclidean) & 2.044118e-02 &                   False \\
      C-means (Euclidean) &       Density Peaks (DTW) & 5.935112e-02 &                   False \\
      Density Peaks (DTW) & Density Peaks (Euclidean) & 1.089868e-01 &                   False \\
    K-medoids (Euclidean) &                   K-shape & 1.367893e-01 &                   False \\
      C-means (Euclidean) &                   K-shape & 1.850786e-01 &                   False \\
      C-means (Euclidean) & Density Peaks (Euclidean) & 2.050779e-01 &                   False \\
            K-means (DTW) &       K-means (Euclidean) & 2.188934e-01 &                   False \\
            K-means (DTW) &                   K-shape & 2.249359e-01 &                   False \\
Agglomerative (Euclidean) &                   K-shape & 3.193606e-01 &                   False \\
Agglomerative (Euclidean) &             K-means (DTW) & 7.882831e-01 &                   False \\
      C-means (Euclidean) &     K-medoids (Euclidean) & 9.768389e-01 &                   False \\
      K-means (Euclidean) &                   K-shape & 9.918929e-01 &                   False \\
\bottomrule
\end{tabular}

%End of latex from pandas
\caption{Pairwise comparison of the algorithms according to the Wilcoxon signed-rank test with a 95\% confidence level with the Holm correction in p value. }
\label{p_values}
\end{table*}



Even though the training stage of the Agglomerative algorithm is faster for some data sizes, it has drawbacks in some applications. R-clustering, as other algorithms based on K-means, can classify new data points easily using the centroids calculated in the training process just by assigning the new instance to the class represented by the nearest centroid. On the contrary,  Agglomerative does not generate any parameter that can be applied to new instances. Therefore, when using Agglomerative to classify new data the whole training process should be repeated with the training data and the new observation.

%\begin{figure*}[ht]
 %   \centering
  %  \includegraphics[width=\linewidth]{pics/cd-diagram-cliques.jpeg}
   % \caption{Critical differences diagram showing the critical differences among the compared algorithms}
    %\Description{diagram showing the algorithms sorted by mean rank and their significant differences in performance.}
    %\label{fig:cd-diagram-cliques}
%\end{figure*}




\subsection{Statistical analysis of the benchmark}
To strengthen the results of the cited benchmark, following recommendations by \cite{garcia2008extension}, we repeat the pairwise comparisons among each of the algorithms in the benchmark, not only with the newly presented method. The results are presented in table \ref{p_values}, that shows which pair of algorithms have significant difference in performance regarding mean rank with a 95\% confidence level. Note that the threshold for the p-value is not 0.05, but it is modified according to the Holm correction to control the family-wise error \cite{demvsar2006statistical}.

The authors of the UCR dataset recommend representing these kinds of comparisons in a critical differences diagram grouping the algorithms within which there is no significant difference. However, the diagram is not very comprehensive in our study due to the high number of resulting groups. In stead, we present the results in table \ref{p_values}, showing significant differences between each pair of algorithms.







%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%  DISCUSION  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Conclusions and future work}
\label{sec:discussion}
We presented R-clustering, a clustering algorithm that uses random convolutional kernels. R-clustering transforms time series into a new data representation, which feeds a K-means algorithm with Euclidean distance. We evaluate the new algorithm following the procedures of a recent clustering benchmark study that uses the UCR archive, the largest public archive of labeled time-series datasets, and state-of-the-art clustering algorithms. R-clustering obtains the first place among all the algorithms evaluated across all datasets using the same evaluation methods as in the study. We also demonstrate the scalability of R-clustering in terms of time series length and dataset size, and show that it becomes the fastest algorithm for large datasets. Finally, following recent recommendations of the machine learning academic community, we strengthen the cited benchmark results with a pairwise statistical comparison of the algorithms included. This statistical analysis and the fact that the code used for generating the results in this paper is publicly available should ease testing future time series clustering algorithms.


%Random Kernels efectiveness
In light of the results, random kernels effectively improve the clustering accuracy of time series. This discovery motivates us to propose future works such as adapting R-clustering for multivariate series, for other type of data like image clustering, or studying the relation between the number of kernels and the performance that could suggest an optimal number of kernels depending on the time series length. %that is, adapting the number of parameters and the data size.

The excellent performance of random kernels has been shown through experimental results rather than theoretical ones. In this sense, we also encourage the academic community to analyze the theoretical aspects of random kernel transformations in more detail. Advances in this direction could account for a better comprehension of the process.

%Limitations




==> zz_otros.tex <==
%%ELBOW METHOD ANALYTICALLY

Finf in which step the decrease or increase is significative

Using mle: https://tminka.github.io/papers/pca/minka-pca.pdf is not possible because it requires number of samples > number of features


